Network Traffic Characteristics of IoT Devices in Smart Homes

Understanding network traffic characteristics of IoT devices plays a critical role in improving both the performance and security of IoT devices, including IoT device identification, classification, and anomaly detection. Although a number of existing research efforts have developed machine-learning based algorithms to help address the challenges in improving the security of IoT devices, none of them have provided detailed studies on the network traffic characteristics of IoT devices. In this paper we collect and analyze the network traffic generated in a typical smart homes environment consisting of a set of common IoT (and non-IoT) devices. We analyze the network traffic characteristics of IoT devices from three complementary aspects: remote network servers and port numbers that IoT devices connect to, flow-level traffic characteristics such as flow duration, and packet-level traffic characteristics such as packet inter-arrival time. Our study provides critical insights into the operational and behavioral characteristics of IoT devices, which can help develop more effective security and performance algorithms for IoT devices.

==> 04c2_packet_based_analysis.tex <==
\subsubsection{Packet Lengths (payload)}

In this subsection we will study the outgoing packet lengths. We will count the payload bytes only.

\begin{figure}[th]
\centering
\subcaptionbox{IoT devices \label{fig:outgoing-pktlens-tcp-iot}}[0.48\linewidth]
    {\includegraphics[width=0.24\textwidth]{plots/fwd_pktlens_tcp_iot.png}}
\hfill
\subcaptionbox{non-IOT devices \label{fig:outgoing-pktlens-tcp-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.24\textwidth]{plots/fwd_pktlens_tcp_noniot.png}}
\caption{Packet lengths (bytes) of outgoing packets of TCP flows.}
\label{fig:outgoing-pktlens-tcp}
\end{figure}

\begin{figure}[th]
\centering
\subcaptionbox{IoT devices \label{fig:outgoing-pktlens-udp-iot}}[0.48\linewidth]
    {\includegraphics[width=0.24\textwidth]{plots/fwd_pktlens_udp_iot.png}}
\hfill
\subcaptionbox{non-IOT devices \label{fig:outgoing-pktlens-udp-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.24\textwidth]{plots/fwd_pktlens_udp_noniot.png}}
\caption{Packet lengths (bytes) of outgoing packets of UDP flows.}
\label{fig:outgoing-pktlens-udp}
\end{figure}

==> 06_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper we analyzed the network traffic characteristics of IoT devices collected on a typical smart home environment consisting of a set of common IoT (and non-IoT) devices. We analyzed the network traffic characteristics of IoT devices from three complementary aspects: remote network servers, flow-level traffic characteristics, and packet-level traffic characteristics.  Our study provided critical insights into the operational and behavioral characteristics of IoT devices, which could have important implications on developing effective security and performance algorithms for IoT devices.

==> 10_additional.tex <==
\section{Additional Figures}
\begin{figure*}[th]
\centering
\subcaptionbox{Flow duration (TCP and UDP) of IoT devices \label{fig:flow_duration_iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_duration_iot.png}}
\hfill
\subcaptionbox{Flow duration (TCP and UDP) of non-IoT devices \label{fig:flow_duration_noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_duration_noniot.png}}
  \caption{Flow duration for IoT and non-IOT devices.}
\label{fig:flow-durations}
\end{figure*}

Figures~\ref{fig:flow_duration_iot} and~\ref{fig:flow_duration_noniot} shows the flow duration of a few representative IoT and non-IoT devices. In these two figures, a flow can be either a TCP or UDP flow. First we note that a large percentage of flows have very short flow durations for all IoT devices. Non-IoT devices also have a large number of flows with short flow durations. However, this percentage is lower in non-IoT devices. Second, we note that a number of IoT devices have a few concentrated flow durations. For example, about $30\%$ of the Cam5 flows have a flow duration of $120$ seconds. In contrast, as we can see from Figure~\ref{fig:flow_duration_noniot} that non-IoT devices do not have this kind of concentrated flow durations. The durations of non-IoT flows are more spread out. 

\begin{figure*}[th]
\centering
\subcaptionbox{Flow size (TCP and UDP) for IoT devices \label{fig:flow-bytes-iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_bytes_iot.png}}
\hfill
\subcaptionbox{Flow size (TCP and UDP) for non-IoT devices \label{fig:flow-bytes-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_bytes_noniot.png}}
\caption{Flow size for IoT and non-IOT devices.}
\label{fig:flow-bytes}
\end{figure*}


Figure~\ref{fig:flow-bytes-iot} shows the amount of traffic of flows of IoT devices. From the figure we can see that most of IoT devices only generate a small amount of traffic. For example, close to $90\%$ of flows of all IoT devices generated less than $10$ bytes of data traffic. Figure~\ref{fig:flow-bytes-noniot} shows the amount of traffic of flows of non-IoT devices. From the figure we can see that, on average, non-IoT devices have larger flows. For example, only less than $70\%$ of flows of all non-IoT devices generated less than $10$ bytes of data traffic.

\begin{figure*}[!h]
%\subcaptionbox{Subcaption A}
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{plots/flowrate_pkts_iot.png}
    \caption{IoT devices}
    \label{fig:flow-rate-pkts-iot}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{plots/flowrate_pkts_noniot.png}
    \caption{Non-IoT devices}
    \label{fig:flow-rate-pkts-noniot}
\end{subfigure}
\caption{TCP+UDP Flow rate (packets/second).}
\label{fig:flow-rate-pkts}
\end{figure*}

\begin{figure*}[!h]
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{plots/flowrate_bytes_iot.png}
    \caption{IoT devices}
    \label{fig:flow-rate-bytes-iot}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{plots/flowrate_bytes_noniot.png}
    \caption{Non-IoT devices}
    \label{fig:flow-rate-bytes-noniot}
\end{subfigure}

\caption{TCP+UDP Flow rate (bytes/second).}
\label{fig:flow-rate-bytes}
\end{figure*}

\begin{figure*}[th]
\centering
\subcaptionbox{IoT devices \label{fig:active-flows-iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/active_flows_iot.png}}
\hfill
\subcaptionbox{non-IOT devices \label{fig:active-flows-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/active_flows_noniot.png}}
\caption{Number of Flows (TCP+UDP) for IoT and non-IOT devices at time intervals.}
\label{fig:active-flows}
\end{figure*}

==> old_files/01_introduction.tex <==
\section{Introduction}
[Points:
1. Globalization of IoT devices, expanding usage
2. Vulnerability, easy to exploit, lack of processing and power
3. Necessary to identify/protect
4. Lots of studies - lack of detailed traffic analysis
]
\\ \\

....

Recent technological advancement enabled us the opportunity to devise and connect smart devices to serve all levels of jobs, from easy to difficult. We use smart thermostats to automatically adjust home or other environments, smart camera and alarm systems to provide a better security, smart sensors and lights to ease daily jobs, and many more to mention. Besides smart home and city environments, lots of IoT devices are being connected in industries and other sectors everyday. Smart cars are evolving, and almost all car manufacturers offer smart head units in their recently released cars. Users can track the location of the car, and perform some basic operations such as start/stop engine, control the air conditioner from the companion mobile app of the car.



With a continuous growth, the number of IoT devices reached 11.7 billion in 2020 which surpassed the number of non-IOT devices for the first time. As more and more devices are connected for different purposes, there will be 30.9 billions of IoT devices in 2025 which will be three times more than non-IoT devices at that time\cite{numberofiot}.

\\ 
\\

\textbf{Many other papers cite the study performed by IHS and supposed to be available on https://ihsmarkit.com/Info/1017/internet-of-things.html but this link does not work, it redirects to a general page.}
\\ 
\\



Typically, IoT devices possess low processing capabilities, limited memory and storage, as well as minimal network protocol support, to prolong battery life. These limitations pose a significant challenge for device manufacturers and engineers in their quest to design complex and comprehensive security measures~\cite{challengessecurigiot}. Also, a continuous demand for the latest and greatest IoT gadgets leads to a competition for manufacturers to produce more devices at an affordable price~\cite{whymanuinsecure}, leaving security implementations out of focus. Furthermore, security patches might not be updated regularly due to irregular release or to a lack of awareness of the users to installation overheads~\cite{iotwildlyinsecure}. These factors ultimately keep a huge number of devices vulnerable. Since IoT devices are connected to the Internet, these vulnerabilities are exposed on the Internet, which attackers could exploit remotely~\cite{hadar2017lightweight}.

IoT systems are deployed in public, private, and corporate spaces, and a significant amount of information is being collected from these environments to make intelligent decisions. This huge amount of information, along with the easy vulnerabilities of the devices, attracts the attackers who want to exploit the IoT systems. In 2016, the massive DDoS attack on Dyn data centers made their DNS service unreachable to users. The attack is performed using Mirai botnets on IoT devices and it took down more than 1200 domains they were supporting, including Amazon, Github, Twitter, Shopify and many other major ones~\cite{dynddos}. Several other attacks emerged afterwards which are not as devastating as the Mirai but still severe.

Paragraph: Recently, a number of studies performed on different countermeasures against these vulnerabilities. We can boradly categorize the work into two directions - identifying an IoT device on the connected network and detecting whether the device is compromised. Both of these research directions utilize the the network traffic of the devices. 

[Link this paragraph to the next one]

There are lots of studies for IoT device recognition or classification which analyze network flows or network packet characteristics of the IoT traffic, but none of them presented a deep analysis on the traffic itself. In this work we are trying to present a detailed analysis of traffic behaviors of some typical IoT devices in a home network as well as some comparisons with non-IoT counterparts.

As we analyze different characteristics of IoT traffic, we have some features related to the traffic flow where some features are related to packet information. We will discuss both of these categories in different sections so that an overall picture of the traffic can be presented. 

==> old_files/02_related_work.tex <==
\section{Related Work}

Several studies are performed by different researchers to identify IoT devices and analyze their characteristics in home networks. 
Mazhar and Shafiq~\cite{mazhar2020characterizing} performed a study on IoT traffic analysis in a home network environment. They unitized flow level summary information gathered from the gateway routers installed in different homes deployed and managed by a home gateway management company. They found that 60\%-90\% of the traffic from IoT devices are connected to Google Cloud and amazon AWS. This is because aside from the devices from google and amazon, most of the other vendors are interested to host their services on third party cloud servers to get rid of maintenance and other overhead. Another observation they mentioned is about the dns query; most of the IoT devices use hard-coded Google DNS servers for various reasons. The researchers also mentioned some adware traffic and unencrypted traffic which are supported by other researchers as well. However, the researchers have access to some of the flow level information only without any details to the packet level information. As some other studies suggest, some packet level information (such as Inter-Arrival times) plays an important role in analyzing IoT behavior~\cite{shahid2018recognition}.

Meidan et al. used IoT traffic data to detect and whitelist IoT devices connected to the current network~\cite{meidan2017detection}. They used selected features from TCP sessions information to train their machine learning model. Doshi et al. presented a model to distinguish normal and attack traffic by using machine learning techniques on different network traffic features~\cite{doshi2018machine}. They used simulated IoT traffic data for their study.

Some device identification works utilize only initial traffic to identify IoT devices. 

Shahid et al. present a study to recognize IoT devices by analyzing first N packets of TCP flows of IoT devices. They only considered the packet size and packet inter-arrival times for those set of packets for their study and classified different IoT devices using machine learning techniques~\cite{shahid2018recognition}. However, their study was in a very limited scope, the network having only four IoT devices with no non-IoT devices.

 Miettinen  and his team worked on IoT device fingerprinting and identification which utilizes the network traffic during the setup phase~\cite{miettinen2017iot}. Ammar et al. present a different approach of identifying IoT devices. Their work uses service discovery and DHCP protocols to collect information about devices during the setup phase, and uses that information in machine learning techniques~\cite{ammar2019network}. 

Sivanathan et al. presented a work on classifying IoT devices based on statistical attributes of their network activity. They extracted several features from the network traffic including activity cycles, remote servers and ports, signaling patterns, and cipher suites to feed into their classifier to classify IoT devices~\cite{sivanathan2018classifying}. Almost all the works use different features from network traffic to perform their study but we could not find any work that gives an insight of what happening inside the network traffic except the last one \textbf{partially does}. Also, some studies use simulated traffic because of lack of publicly available IoT traffic dataset. Our aim for this work is to provide a thoroughly detailed study of the IoT traffic itself so that it helps other researchers how different features can be extracted and which features contribute the most toward device detection or behavior analysis and why. 

==> old_files/03_traffic_collection_0822.tex <==
%\section{Traffic Collection}
%\subsection{Device and Network Setup}
\section{Network Setup and Traffic Collection}
\subsection{Devices and Network Setup}
Figure~\ref{fig:network1} illustrates the setup of the network testbed in a home environment, from which we collect the network traffic used in this study. This network comprises a variety of $10$ IoT devices as well as a number of non-IoT devices (see Table~\ref{table:1}), which reflects a typical network setup in a smart home environment. All devices are connected to a Netgear AC3200 Wi-Fi router. The Netgear router is connected to a Technicolor DOCSIS $3$ cable modem which is a WiFi router as well. We sometimes connect mobile phone to the Technicolor router to test some cross-network traffic flow.

%%Figure \ref{fig:network1} presents our testbed setup in a home environment. This setup comprises a variety of %%IoT devices as well as some non-IoT devices which reflects a typical representation of a smart home network. %%All devices are connected to a Netgear AC3200 WiFi router. The router is connected to the cable modem to %%connect to the Internet.

%Table \ref{table:1} shows the list of MAC and IP addressess of the devices connected in the network. 
This home network contains three pairs of security cameras. A pair of Logitech Circle-2 cameras are placed at different outdoor locations; two indoor cameras (Wyze and Eufy Indoor) are placed at the same location at the front porch; and another pair of indoor cameras (Eufy pan/tilt and LittleElf) are placed inside the living room. This combination of similar cameras at different locations and different cameras at the same location helps us to observe the traffic behavior of these security cameras from different angles. This home network also contains three smart plugs from three different manufacturers and an HP printer. Two laptops, two smart phones and an iPad, representing non-IoT devices, are also connected with the Netgear Wi-Fi router. 

We have some observations on behaviors of different devices when they operate through the mobile apps. Logitech cameras (Cam1 and Cam2) always send the data to the server whenever an event happens or we watch the live stream through the mobile app. Wyze (Cam3), Eufy (Cam4 and Cam5), and LittleElf (Cam6) cameras send the traffic to server when there is an event, but they send the traffic directly to the mobile for a live stream on the mobile app if the mobile is connected to the DOCSIS router or the Netgear router (need some explanation). For playback of previous videos, the Wyze and Eufy cameras still send the traffic directly to the mobile while LittleElf camera sends the traffic to server which comes to the mobile from the server. (Here server means the remote server the camera is connected to.) Similar behavior happens in case of smart plugs and bulb. When the mobile phone is connected on the same network (the Netgear router) the app sends the signal to the device directly, otherwise, the signal goes from the app to the device trough the server.

The Logi Circle-2 cameras do not have local storage, so they are not capable of continuous recording. All other cameras have local SD card storage where they store 24/7 recording. All cameras have motion detection enabled. When any motion is detected, a camera will upload the footage to the server and send a notification through the mobile app where the camera is connected and configured. Also, all the cameras have live view feature which enables a user to view the live video through the mobile app. 

All devices are assigned with static IP addresses on the router so that we can keep track of their traffic with IP addresses in addition to their MAC addresses. Table~\ref{table:1} shows these IoT and non-IoT devices used in this study, including their corresponding MAC and IP addresses. In the table, the column  "Device" indicates the manufacture and type of the device. For each device, we also provide an "Alias Name", which is used to refer to the device throughout the paper to simplify our exposition.

The Netgear Wi-Fi router is flushed with OpenWrt firmware~\cite{openwrt} to ease the collection of network traffic on the home network. A few software packages are installed on the router to help capture network traffic from all the connected devices. A Unix cron job runs the tcpdump tool on the router, which captures the traffic from all the devices and saves the captured traffic to an attached 512GB USB flash drive. The cron job runs tcpdump for each device separately and restarts the tcpdump processes at midnight. In this way we obtain a separate trace file every $24$ hours for each device while keeping the file sizes within a reasonable limit. We note that we handle the three smart plugs differently from other devices. Given the small amount of the traffic generated by the plugs, their daily traffic is collected together in a single pcap file.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/network1.png}
    \caption{Smart home network setup}
    \label{fig:network1}
\end{figure}

\begin{table*}[htbp]
\renewcommand{\arraystretch}{1.5}
\caption{Connected Devices in Smart Home Network}
\label{table:1}
\centering
\begin{tabular}{|l|l|l|l|l|}
  \hline
  Device & Alias Name & Category & MAC Address & IP Address \\
  \hline
  \multirow{2}{*}{Logitech Circle-2} & Cam1 & \multirow{10}{*}{IoT} & 44:73:D6:0C:36:AD & 192.168.1.158 \\
  \cline{2-2} \cline{4-5}
  & Cam2 & & 44:73:D6:09:BD:C9 & 192.168.1.186 \\
  \cline{1-2} \cline{4-5}
  Wyze Cam & Cam3 & & 2C:AA:8E:95:F3:18 & 192.168.1.228 \\
  \cline{1-2} \cline{4-5}
  Eufy Indoor Cam & Cam4 & & 8C:85:80:38:98:AF & 192.168.1.182 \\
  \cline{1-2} \cline{4-5}
  Eufy Pan and Tilt & Cam5 & & 8C:85:80:3A:12:B4 & 192.168.1.131 \\
  \cline{1-2} \cline{4-5}
  LittleElf Cam & Cam6 & & 0C:8C:24:61:50:29 & 192.168.1.168 \\
  \cline{1-2} \cline{4-5}
  Epicka Smart Plug & Plug1 & & DC:4F:22:0E:C6:36 & 192.168.1.127 \\
  \cline{1-2} \cline{4-5}
  Amazon Smart Plug & Plug2 & & F8:54:B8:25:AA:C9 & 192.168.1.204 \\
  \cline{1-2} \cline{4-5}
  Unbranded Smart Plug & Plug3 & & DC:4F:22:16:11:F1 & 192.168.1.235 \\
  \cline{1-2} \cline{4-5}
  HP Envy Printer & Printer & & 94:57:A5:0C:5B:66 & 192.168.1.248 \\
  \hline
  HP Elitebook  & Laptop1 & \multirow{5}{*}{non-IoT} & AC:FD:CE:01:7C:9B & 192.168.1.105 \\
  \cline{1-2} \cline{4-5}
  Apple iPhone X & iPhone & & 34:08:BC:DE:E9:7E & 192.168.1.203 \\
  \cline{1-2} \cline{4-5}
  Apple iPad & iPad & & E8:8D:28:14:82:30 & 192.168.1.125 \\
  \cline{1-2} \cline{4-5}
  Samsung S20 & Android & & 16:05:DD:78:5F:20 & 192.168.1.215 \\
  \cline{1-2} \cline{4-5}
  HP ZBook & Laptop2 & & CC:2F:71:3B:0E:DE & 192.168.1.247 \\
  \hline
\end{tabular}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Data Pre-processing}
The USB flash drive has different folders for each device and daily traffic is stored in separate pcap files. We copy those pcap files from the router to a laptop for processing. We use CICFlowMeter\cite{cicflowmeter} to extract the traffic flows from the pcap files. The output of the CICFlowMeter is a csv file which contains more than eighty features. The necessary features are imported into MySQL database to perform some more processing work. \textbf{The CICFlowmeter flows include both TCT and UDP streams.} We perform all flow-based analysis based on the data stored on MySQL database.

We use tshark tool to handle pcap files for different types of data analysis. Separating TCP and UDP flows, separating a host traffic from a combined traffic, getting list of outgoing hosts or ports are some examples of usage of tshark in our work. For packet based analysis, we extracted TCP and UDP flows from pcap files and imported the data into MySQL database. We performed MySQL queries to calculate outgoing bytes or packets in different times and many other operations. We used IP packet length for packet level analysis.

==> old_files/04a_remote.tex <==
\subsection{Remote Servers}
% \section{Traffic Analysis}
% In this section, we will present the analysis of the network traffic collected from the activities of different devices. We will analyze the traffic in three different ways: Outside interactions, Packet-level analysis, and Flow-level analysis.
% %%%%%%%%%%%%%%%%%   Outgoing servers and ports  %%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Outgoing hosts and ports distribution}

% \input{04a_host_port_analysis}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Flow-based Analysis}

% \input{04b_flow_based_analysis}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Packed-based Analysis}

% \input{04c_packet_based_analysis}


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.47\textwidth]{plots/outgoing_ports_3}
%     \caption{Number of different outgoing ports.}
%     \label{fig:outgoing_ports}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.47\textwidth]{plots/outgoing_ips_3}
%     \caption{Number of different outgoing IP addresses.}
%     \label{fig:outgoing_ips}
% \end{figure}

% \begin{figure*}[th]
%   \centering
%   \subfigure
%   {
%     \includegraphics[width=0.4\paperwidth]{plots/outgoing_hosts_3.png}
%     \label{fig:asn_theta_0}
%     \subcaption{Fig a}
%   }
%   \subfigure
%     {
%       \includegraphics[width=0.4\paperwidth]{plots/outgoing_ports_3.png}
%       \label{fig:asn_theta_1}
%       \subcaption{Fig B}
%     }
%     \caption{Average number of required observations when $H_1$ is true
%     ($\beta = 0.01$)}
%     \label{fig:asn}
% \end{figure*}

\begin{figure*}[!h]
\begin{subfigure}
    \includegraphics[width=0.4\paperwidth]{plots/outgoing_hosts_3.png}
    % \caption{Outgoing hosts}
    \label{fig:outgoing_hosts}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.4\paperwidth]{plots/outgoing_ports_3.png}
    % \caption{Outgoing ports}
    \label{fig:outgoing_ports}
\end{subfigure}
\caption{Outgoing hosts and ports}
\label{fig:outgoing_hosts_and_ports}
\end{figure*}
% \FloatBarrier

% \begin{figure*}[!ht]
%     %  \captionstyle{centerlast}
%      \begin{minipage}[l]{1.0\columnwidth}
%          \centering
%          \includegraphics[width=0.9\textwidth]{plots/outgoing_hosts_3.png}
%          \caption{AAA}\label{fig:AAA}
%      \end{minipage}
%      \hfill{}
%      \begin{minipage}[r]{1.0\columnwidth}
%          \centering
%          \includegraphics[width=0.9\textwidth]{plots/outgoing_ports_3.png}
%          \caption{BBB}\label{fig:BBB}
%      \end{minipage}
% \end{figure*}

% \begin{figure*}[t]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.8\linewidth]{plots/outgoing_hosts_3.png}  
%   \caption{Put your sub-caption here}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.8\linewidth]{plots/outgoing_ports_3.png}  
%   \caption{Put your sub-caption here}
%   \label{fig:sub-second}
% \end{subfigure}
% \caption{Put your caption here}
% \label{fig:fig}
% \end{figure*}


% \begin{figure}[htbp]
%     % \centering
%     \subfigure[Cap 1]{
%     \includegraphics{plots/outgoing_hosts_3}
%     \caption{Number of different outgoing hosts.}
%     \label{fig:outgoing_hosts}
%     }
%     \subfigure[caption 2]{\label{...}
%     \includegraphics{plots/outgoing_ports_3}\hspace{1em}
%     \includegraphics{img1-b}\hspace{1em}
%     \includegraphics{img1-c}
%     }
% \caption{Outgoing hosts and ports.}
% \label{fig:outgoing_hosts_ports}
% \end{figure}

\begin{table*}[t]
\centering
\caption{Outgoing ports and hosts for IoT devices}
\label{table:outgoing_host_port}
\begin{tabular}{|c|c|c|c|c|}
% \begin{tabularx}{1\linewidth}{
%   | >{\raggedright\arraybackslash}X 
%   | >{\raggedright\arraybackslash}X   %centering, raggedleft
%   | >{\raggedright\arraybackslash}X
%   | >{\raggedright\arraybackslash}X
%   | >{\raggedright\arraybackslash}X |
%   }
  \hline
   
  Device & TCP Ports & UDP Ports (Up to most frequent 4) &  TCP Hosts & UDP Hosts (Up to most frequent 4) \\
  \hline
  \multirow{2}{*}{Cam1/Cam2} & 443 & 137, 123, 53, 67 & amazonaws.com & pool.ntp.org, Router \\
  & &  & & arpnetworks.com, latt.net \\

  \hline
  \multirow{2}{*}{Cam3} & 443, 8443, 8883 & 10001, 53, 137, 123 & amazonaws.com & homeassurednow.com, ip-192-99-160.net \\
  &  &  &  &   ip-147-135-36.us, Router \\

  \hline
  \multirow{2}{*}{Cam4} & 443 & 32100, 8006, 53, 15064 & amazonaws.com & amazonaws.com, eufylife.com \\
  &  &  &  & Router, comcast.net \\

  \hline
  \multirow{2}{*}{Cam5} & 443 & 32100, 26807, 25249, 53 & amazonaws.com & amazonaws.com, iPhone (local) \\
  &  &  &  & Router, 114dns.com \\

  \hline
  \multirow{2}{*}{Cam6} & 19000, 19001 & 137, 53, 123, 68 & amazonaws.com & nist.gov, Router \\
  &  &  &  & dns.google, colorado.edu \\

  %cline
  \hline
  \multirow{1}{*}{Plug1} & 1883, 80, 36020 & 6666, 137, 67 & amazonaws.com & 255.255.255.255, Router \\

  \hline
  \multirow{1}{*}{Plug2} & 443 & 137, 53, 67 & amazonaws.com & amazonaws.com, Router, amazon.com \\
  \hline
  \multirow{2}{*}{Printer} & 443, 5222 & 9930, 5353, 138, 53 & amazonaws.com & amazonaws.com, Router \\
  & 5357, 58998 & & laptop2 (local), 1e100.net & laptop2 (local), Router \\
  \hline
\end{tabular}
\end{table*}

In this section, we will show how the IoT devices communicate with outside world. We will show the total number of TCP and UDP hosts and ports the devices connected to for one day. A weekly analysis of the communicating hosts and ports for the devices will be presented on the second part of this section.


\subsubsection{Outgoing hosts and ports for one day}
Fig.~\ref{fig:outgoing_hosts_and_ports} shows a comparative representation of outgoing hosts and ports for IoT and non-IoT devices for a one-day traffic. As anticipated, IoT devices communicate with a limited number of hosts as part of their regular work. As the devices are connected to a server for their status update and other activities, they regularly send packets to the server and maintains longer TCP sessions (we have more detailed analysis on flows and sessions in later section). Some devices follow precise pattern of communication with some servers. For example, the amazon plug sends packets to updates.amazon.com and api.amazon.com fourteen times a day, the printer communicates eighteen times to hermes.instantink.com \footnote{HP instant ink is a monthly subscription which keeps track of the current ink level on the printer and ships cartridges automatically whenever needed.} a day. The devices maintain these connections to get regular updates from their servers. Smart bulb and plugs do not have any UDP connections while cameras maintain some UDP connections with different time servers. The Fig.~\ref{fig:outgoing_hosts_and_ports} also shows that the printer has a lot of different outgoing ports. Inspecting the traffic more carefully suggests that the printer connects to laptops with different TCP ports which results in big number of different ports. Similarly, iPhone has a big number of ports; inspecting those ports reveals that iPhone is connected to youtube and facebook using different port numbers. 

Table~\ref{table:outgoing_host_port} shows a list of most frequent TCP/UDP hosts and ports for IoT devices. We see that IoT devices mainly use port 443 for their TCP connections and rarely use port 80 which is very common for non-IoT devices since users browse different websites using port 80 in addition to port 443. Some IoT devices use port numbers other than 443, for instance, Cam6 uses ports 19000 and 19001, but inspecting the traffic looks like they use these ports deliberately to communicate their server instead of regular 443 port. We notice from the table that Cam5 has lots of UDP connections with iPhone; this is because when we go to live view of the camera in mobile app, the video is sent directly to the mobile using UDP connection. The outgoing connections for non-IoT devices are much more compared to IoT devices and unpredictable as they are operated by users. They perform a wide range of TCP and UDP connections with outside hosts for different purposes. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Weekly analysis of outgoing hosts and ports}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.47\textwidth]{plots/weekly_hosts_cam1.png}
%     \caption{Weekly hosts for Cam1.}
%     \label{fig:weekly_hosts_cam1}
% \end{figure}

\begin{figure*}[!h]
\begin{subfigure}
    \includegraphics[width=0.4\paperwidth]{plots/weekly_hosts_cam1.png}
    % \caption{Weekly hosts Cam1}
    \label{fig:outgoing_hosts_cam1}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.4\paperwidth]{plots/weekly_hosts_laptop2.png}
    % \caption{Weekly hosts Laptop2}
    \label{fig:outgoing_hosts_laptop2}
\end{subfigure}
\caption{Weekly hosts Cam1 and Laptop2.}
\label{fig:weekly_hosts_cam1_laptop2}
\end{figure*}

Fig.~\ref{fig:weekly_hosts_cam1_laptop2} shows outgoing hosts for a representative IoT and non-IoT device. For Cam1, we do not see any change in the number of TCP hosts throughout the week, the device is connecting only to amazonaws.com with TCP protocol. However, it has new and different numbers of external UDP servers on different days. Most of these hosts are connections to NTP (Network Time Protocol) servers and DNS queries. All IoT devices show similar behavior regarding TCP connections, however, the plugs and smart bulb connects only a few external hosts and they are not NTP servers or DNS servers. On the other hand, the laptop communicates a large number of TCP and UDP hosts and this remains consistent throughout the period. This is because laptop uses different applications which connect to different external servers and ports, and also the user browses different websites for different purposes. Other non-IoT devices show similar big number of external connections.

==> old_files/4b_flow_level.tex <==
We will provide some flow based analysis in this section. We use CIC Flowmeter to extract TCP and UDP flows from pcap traces. This tool generates a csv file which is imported into a MySQL database. The data in the MySQL database is used for different types of analysis in this section.

\subsubsection{Inter Arrival Time (IAT)}
The term \textbf{Inter Arrival Time (IAT)} means the duration between two consecutive outgoing or incoming packets. For example, when we say outgoing Inter Arrival Time, it means how long it takes to send the next packet after a packet is sent in the same direction for a flow. The CIC Flowmeter counts the inter arrival times between packets separately for incoming and outgoing packets for each flow. We are using the total outgoing IATs in flows for the analysis in this section.

\begin{figure*}[th]
\centering
\subcaptionbox{IATs for IoT devices \label{fig:outgoing-iat-iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/fwd_iat_iot.png}}
\hfill
\subcaptionbox{IATs for non-IOT devices \label{fig:outgoing-iat-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/fwd_iat_noniot.png}}
\caption{Outgoing Packet IATs for IoT and non-IOT devices.}
\label{fig:outgoing-iat}
\end{figure*}

Fig.~\ref{fig:outgoing-iat} shows the Inter Arrival Times between outgoing packets in flows for different devices. We see from Fig.~\ref{fig:outgoing-iat-iot} that IoT devices have a longer range of Inter Arrival Times. Most of the devices has higher IATs. For instance, the Plug1 has longer than 10000 milliseconds IATs for most of the packets in outgoing flows. The printer has a relatively smaller IATs but still more than $70$ percent have IATs longer than 100 milliseconds. On the other hand, Inter Arrival Times are concisely distributed in case of non-IoT devices. We find from Fig.~\ref{fig:outgoing-iat-noniot} that almost all the devices have an IAT range smaller than 100 milliseconds for about $80$ percent cases. Quantitative analysis shows that all non-IoT devices have the smallest IAT as 5 microseconds and the highest IAT ranging from 118.94 (Laptop1) to 119.92 (Laptop2) seconds. On the other hand, IoT devices have Inter Arrival Times ranging from 6 microseconds (Cam3) to 119.79 seconds (Printer) with most of them are limited to 60 seconds while only the printer has the highest IAT.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[th]
    \centering
    \includegraphics[width=0.47\textwidth]{plots/max_iat.png}
    \caption{Max outgoing IAT for different devices}
    \label{fig:max-iat}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Inter-Flow Time}
In this section, we will analyze how often a device communicate with external hosts. The inter-flow time is calculated as the duration between the starting time of two consecutive outgoing flows for for a device.   

\begin{figure*}[th]
\centering
\subcaptionbox{IFT for IoT devices \label{fig:interflow_iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/interflow_iot.png}}
\hfill
\subcaptionbox{IFT for non-IOT devices \label{fig:interflow-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/interflow_noniot.png}}
\caption{Inter-Flow Time for IoT and Non-IoT devices.}
\label{fig:interflow}
\end{figure*}

% bulb: 0-125: 32/48/88(seconds)->50(times)  72->48
% cam1: 0-120: 58->85, 57->53, 62->82 63->49
% cam2: 0-146: 2->67, 3->77, 117->64, 118->61
% cam3: 0-155: 0->3053, 1->316, 114, 107
% cam4: 0-237 then 1427: 0->6364, 379, 60->289, 61->166: all are 1 after 64
% cam5: 0-61: 0->11962, 1098, 169, 109, 60->323, 61->199
% cam6: 0-165: 0->93, 126->501
% plug1: 0-123: 120->31, 
% plug2: 0-160: 102->186, 121-> 209, 150->195
% plug3: 0-124: similar to plug1
% printer: 0-22: 5-10->1700+, 6->1963

% laptop1: 0-167, then 7331,7672: all with frequency 1, 0->5318, 1->1807, 2->854, ... all 1 starting at 66
% laptop2: 0-24: 0->55548, then decreasing 
% iphone: 0-855, then 6862: all 1 or 2 after 151: 0->37722, 1-> 2000, then decreasing
% ipad: : 0-1820: 0->4882, 1-> 1103 then decreasing. Most of them are 1, sometimes 2 or 3 from 61
% android: 0-900, then 2358, then 6560. 0->8880, 1-> 2603, then decreasing, all are 0 or 1 after 151

Fig.~\ref{fig:interflow} shows the Interflow times for different devices. The x-axis is the interflow times in seconds and y-axis is their frequency distributions in CDF. We can see from Fig.~\ref{fig:interflow_iot} that most of the interflow times are distributed within $30$ to $100$ seconds while most of the interflow times are concentrated near $0$ for the non-IoT devices. A detailed inspection on the interflow times and frequencies shows that the printer has the lower variation on the interflow times ($0$ to $22$ seconds, and most of those are between $5$ and $10$ seconds. Cam5 and Cam5 have most of the interflow times at $0$ seconds, and the remaining devices have a lower frequency near $0$ and have linear growth to their maximum interflow times. On the other hand, all non-IoT devices have more than $70$\% of their interflow times at $0$ seconds except Laptop1 which has almost $55$\%. All of the non-IoT devices get more than $90$\% interflow times within $11$ seconds. This gives us an impression that non-IoT devices have more flows within a short period of time which IoT devices take longer time to establish a flow after a flow is established.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Concurrent Flows}
In this section we will analyze concurrent flows for different devices. Concurrent flow means how many flows exist at the same time for a device.

\begin{figure*}[th]
\centering
\subcaptionbox{Concurrent Flows for IoT devices \label{fig:concurrent_iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/concurrent_iot.png}}
\hfill
\subcaptionbox{Concurrent Flows for non-IOT devices \label{fig:concurrent_noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/concurrent_noniot.png}}
\caption{Concurrent Flows for IoT and non-IOT devices.}
\label{fig:concurrent-flows}
\end{figure*}

% bulb: 2: 2 flows -> 4 times
% cam1: 2: 2->8, 3->3
% cam2: 2-3: 2->4, 3->4
% cam3: 2-12: 2/581, 3/796, 4/62, ...12/1
% cam4: 2-20: 2/151, 3/241, 6/858, ....20/1
% cam5: 2-17: 2/491, 3/541, 6/1208, ...17/2
% cam6: 2-7: 2/40, 7,2,2,2,2,1
% plug1: 2: 2/1
% plug2: 2-4: 34,3,2
% plug3: 2: 2/9
% printer: 2-10: 2/119, 29,11,....1

% laptop1: 2-31: 2/1098,3/408,.......1
% laptop2: 2-100: 2/9912, 3767,1630,......2
% iphone: 2-132: 2/3883, 3/1099, ............1
% ipad: 2-25: 2/588, 363,190,........1
% android: 2-45: 2/1714, 601,356,.............1

Fig.~\ref{fig:concurrent-flows} shows the number of concurrent flows for IoT and non-IoT devices. We see from Fig.~\ref{fig:concurrent_iot} that IoT devices have less than $5$ concurrent flows for about $90$\% or more cases. We see some more number of flows for Cam5, however, the overall number of concurrent flows is very limited. On the other hand, non-IoT devices have some bigger number of concurrent flows, for instance, we found more than $100$ concurrent flows in the iPhone traffic. Most of the non-IoT traffic has $5$ to $10$ concurrent flows in general.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Flow Durations}
In this section we will analyze concurrent flow durations for combined TCP and UDP flows for different devices in both incoming and outgoing directions. As discussed earlier, flows are either terminated by FIN packets or the timeout periods. And, since the maximum timeout is set as 120 seconds, flow durations can have a maximum duration of 120 seconds. We have grouped the durations for each second, i.e., 0 to 1 second, 1 to 2 seconds and so on and combined the total number of flows having that duration in the presented graphs.

\begin{figure*}[th]
\centering
\subcaptionbox{Flow durations for IoT devices \label{fig:flow_duration_iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_duration_iot.png}}
\hfill
\subcaptionbox{Flow durations for non-IoT devices \label{fig:flow_duration_noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_duration_noniot.png}}
\caption{Flow durations for IoT and non-IOT devices.}
\label{fig:flow-durations}
\end{figure*}

Fig.~\ref{fig:flow-durations} shows a comparative study on flow durations for IoT and non-IoT devices. The printer has most of the flows less than one second long. On the other hand, the Plug1 has most of the flows with duration 60 seconds and 119 seconds. Other IoT devices have flow durations concentrated at some points. We see from Fig.~\ref{fig:flow_duration_noniot} that flow durations of non-IoT devices are not concentrated at any specific point like IoT devices do, rather, they are distributed all over different durations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Flow Size}
In this section we will analyze the flow size for combined TCP and UDP flows for different devices in both incoming and outgoing directions. We grouped the flow sizes by number of kilobytes and how many flows are there for each kilobyte.

\begin{figure*}[th]
\centering
\subcaptionbox{Flow size for IoT devices \label{fig:flow-bytes-iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_bytes_iot.png}}
\hfill
\subcaptionbox{Flow size for non-IoT devices \label{fig:flow-bytes-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/flow_bytes_noniot.png}}
\caption{Flow size for IoT and non-IOT devices.}
\label{fig:flow-bytes}
\end{figure*}

Fig.~\ref{fig:flow-bytes} shows a comparative study on flow sizes for IoT and non-IoT devices. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Hourly Outgoing Number of Packets}
In this section we will present a quantitative analysis of outgoing packets per hour. We have sum up total number of outgoing (TCP + UDP) packets per hour for a $24$ hour duration.

\begin{figure*}[th]
\centering
\subcaptionbox{Hourly number of packets for IoT devices \label{fig:hourly-outgoing-pkts-iot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/hourly_outgoing_pkts_iot.png}}
\hfill
\subcaptionbox{Hourly number of packets for non-IoT devices \label{fig:hourly-outgoing-pkts-noniot}}[0.48\linewidth]
    {\includegraphics[width=0.48\textwidth]{plots/hourly_outgoing_pkts_noniot.png}}
\caption{Hourly number of packets for IoT and non-IOT devices.}
\label{fig:hourly-num-pkts}
\end{figure*}

Fig.~\ref{fig:hourly-num-pkts} shows a comparative study on outgoing number of bytes per hour for IoT and non-IoT devices. We see from the figures that some of the IoT devices (bulb, plug, printer) have almost steady number of outgoing packets in contrast to the cameras which have more unpredictable traffic. This is expected because cameras create and send a video to the server when a motion is detected. On the other hand, the non-IoT devices have completely unpredictable traffic pattern throughout the day and sometimes those are idle or disconnected resulting no traffic. 


